Model Primitive Hierarchical Lifelong Reinforcement Learning

Learning interpretable and transferable subpolicies and performing task decomposition from a single, complex task is difficult. Some traditional hierarchical reinforcement learning techniques enforce this decomposition in a top-down manner, while meta-learning techniques require a task distribution at hand to learn such decompositions. This paper presents a framework for using diverse suboptimal world models to decompose complex task solutions into simpler modular subpolicies. This framework performs automatic decomposition of a single source task in a bottom up manner, concurrently learning the required modular subpolicies as well as a controller to coordinate them. We perform a series of experiments on high dimensional continuous action control tasks to demonstrate the effectiveness of this approach at both complex single task learning and lifelong learning. Finally, we perform ablation studies to understand the importance and robustness of different elements in the framework and limitations to this approach.

==> figures/mphrl_ppo_single_task.tex <==
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}

\begin{axis}[
xlabel={Tasks},
ylabel={Timesteps ($\times 10^6$)},
xmin=-0.0175, xmax=0.3675,
ymin=0, ymax=30,
xtick={0.05,0.3},
xticklabels={L-Maze,D-Maze},
tick align=outside,
tick pos=left,
x grid style={white!69.01960784313725!black},
ymajorgrids,
y grid style={white!69.01960784313725!black},
legend cell align={left},
legend entries={{MPHRL},{PPO}},
legend style={at={(0.03,0.97)}, anchor=north west, draw=white!80.0!black}
]
\addlegendimage{ybar,ybar legend,fill=color0,draw opacity=0,fill opacity=0.5};
\draw[fill=color0,draw opacity=0,fill opacity=0.5] (axis cs:0,0) rectangle (axis cs:0.05,9.5);
\draw[fill=color0,draw opacity=0,fill opacity=0.5] (axis cs:0.25,0) rectangle (axis cs:0.3,24.5);
\addlegendimage{ybar,ybar legend,fill=color1,draw opacity=0,fill opacity=0.5};
\draw[fill=color1,draw opacity=0,fill opacity=0.5] (axis cs:0.05,0) rectangle (axis cs:0.1,7.9);
\draw[fill=color1,draw opacity=0,fill opacity=0.5] (axis cs:0.3,0) rectangle (axis cs:0.35,13.4);
\path [draw=white!41.17647058823529!black, semithick] (axis cs:0.025,9.1)
--(axis cs:0.025,9.9);

\path [draw=white!41.17647058823529!black, semithick] (axis cs:0.275,22.4)
--(axis cs:0.275,26.6);

\path [draw=white!50.19607843137255!black, semithick] (axis cs:0.075,7.2)
--(axis cs:0.075,8.6);

\path [draw=white!50.19607843137255!black, semithick] (axis cs:0.325,12)
--(axis cs:0.325,14.8);

\addplot [semithick, white!41.17647058823529!black, mark=-, mark size=5, mark options={solid}, only marks, forget plot]
table {%
0.025 9.1
0.275 22.4
};
\addplot [semithick, white!41.17647058823529!black, mark=-, mark size=5, mark options={solid}, only marks, forget plot]
table {%
0.025 9.9
0.275 26.6
};
\addplot [semithick, white!50.19607843137255!black, mark=-, mark size=5, mark options={solid}, only marks, forget plot]
table {%
0.075 7.2
0.325 12
};
\addplot [semithick, white!50.19607843137255!black, mark=-, mark size=5, mark options={solid}, only marks, forget plot]
table {%
0.075 8.6
0.325 14.8
};
\path [draw=black, fill opacity=0] (axis cs:0,0)
--(axis cs:0,30);

\path [draw=black, fill opacity=0] (axis cs:1,0)
--(axis cs:1,30);

\path [draw=black, fill opacity=0] (axis cs:-0.0175,0)
--(axis cs:0.3675,0);

\path [draw=black, fill opacity=0] (axis cs:-0.0175,1)
--(axis cs:0.3675,1);

\end{axis}

\end{tikzpicture}
